ASC me to Do Anything: Multi-task Training for Embodied AI

Embodied AI has seen steady progress across a diverse set of independent tasks. While these varied tasks have different end goals, the basic skills required to complete them successfully overlap significantly. In this paper, our goal is to leverage these shared skills to learn to perform multiple tasks jointly. We propose Atomic Skill Completion (ASC), an approach for multi-task training for Embodied AI, where a set of atomic skills shared across multiple tasks are composed together to perform the tasks. The key to the success of this approach is a pre-training scheme that decouples learning of the skills from the high-level tasks making joint training effective. We use ASC to train agents within the AI2-THOR environment to perform four interactive tasks jointly and find it to be remarkably effective. In a multi-task setting, ASC improves success rates by a factor of 2x on Seen scenes and 4x on Unseen scenes compared to no pre-training. Importantly, ASC enables us to train a multi-task agent that has a 52% higher Success Rate than training 4 independent single task agents. Finally, our hierarchical agents are more interpretable than traditional black-box architectures.

==> macros/macros.tex <==

\newcommand{\supp}[1]{\sethlcolor{green}\hl{#1}}

\renewcommand{\supp}[1]{#1}

\newcommand{\todo}[1]{\sethlcolor{red}\hl{#1}}


\newcommand{\eqnref}[1]{Eq.~\ref{#1}\xspace}

\newcommand{\algref}[1]{Alg.~\ref{#1}\xspace}


==> sections/1_intro_old.tex <==
\section{Introduction}

% bring up single task vs. multiple tasks.
Embodied AI (E-AI) researchers have long sought to develop agents that can perform numerous complex tasks within visual environments -- tasks that require navigating around an environment, interacting with objects that lie within it, following instructions and engaging in dialogue with humans in order to answer queries, ask for clarification and provide alerts. While steady progress has been made towards this ambitious goal, particularly in simulated worlds~\cite{Shen2020iGibsonAS,savva2019habitat,Kolve2019AI2THORAn,Xiang2020SAPIENAS,Gan2020ThreeDWorldAP}, most work today focuses on training agents to perform a single task.

% mention about the single task in the E-AI and bring up the questions.
Several individual E-AI tasks have been developed over the past few years, ranging from navigation-centric ones such as point goal~\cite{Anderson2018OnEO} and object goal navigation~\cite{Batra2020ObjectNavRO}, instruction following~\cite{anderson2018vision,ALFRED20}, question answering~\cite{gordon2018iqa,embodiedqa}, tasks incorporating both visual and aural sensing~\cite{Gan2020LookLA}, tasks involving object interaction~\cite{Shen2020iGibsonAS,Zeng2021PushingIO,Zhu2017VisualSP}, multi-agent collaboration~\cite{Jain2019TwoBo}, rearrangement~\cite{Batra2020RearrangementAC,Weihs2021VisualRR} and object manipulation~\cite{Xiang2020SAPIENAS,Ehsani2021ManipulaTHORA}. Evidence across this large body of research suggests that: (a) Present day learning algorithms are very inefficient -- perfecting simpler tasks such as point goal navigation can require more than a billion frames of experience~\cite{Wijmans2020DDPPOLN}, (b) The best performing methods are not as effective for long horizon tasks as well as tasks that involve rich interactions with the world and larger action spaces~\cite{Weihs2021VisualRR}, and (c) As tasks get more complex, the generalization capability of these methods to unseen environments is quite poor~\cite{ALFRED20}. How do we make the leap to developing effective multi-task E-AI agents, when training single task ones is currently so challenging?

% talk about prior multi-task learning, especially on EAI. point out there limitations.
There has been more interest in training multi-task E-AI agents with goal specified via natural language \cite{andreas2017modular, shu2017hierarchical, chaplot2019embodied}. The compositional structure of language allows matches the compositional nature of embodiment tasks, which allows generalization across different tasks. For example, given two different tasks ``\textit{put a plunger in cabinate}.'' and ``\textit{what is the color of plunger?}'', the agent requires to ``\textit{find plunger}'' first, which is essentially an object navigation task. An agent trained on all the tasks is arguably more robust compared to trained on single tasks. However, prior work in training multi-task agents is either operate in a grid-world environment \cite{andreas2017modular}, or embodiment environment with limited complexities, such as mine-craft to stack blocks \cite{shu2017hierarchical} or ViZDoom with single room with 5 objects \cite{chaplot2019embodied}. 
% some argument might be: Should we focus on learning skill in a incremental way? or just multi-tasking?  for the first argument, there are a lot of work, how do we differentiate our from others in this? 
% make this a few sentence. Similar to pre-training, this allows to learn fundamental skill. 
% \jl{This section should be changes. we should mention why there is no agent in complex multi-tasking environments. 1) different tasks require different sensors, version of environments. 2) there is lack of api that connecting different task (this is a little bit tricky since similar ideas has explored in much simpler tasks). We took the first step to}

% Across the landscapes of computer vision and natural language processing (NLP), pre-training models using large amounts of data has been a very effective mechanism to arrive at strong models for downstream tasks. In computer vision, pre-training on the ImageNet dataset and fine-tuning on single as well as multi downstream tasks has become the de facto standard~\cite{Simonyan2015VeryDC}. In NLP, generative pre-training on large language corpora has led to the development of highly capable few-shot learners~\cite{gpt3}. In the vision and language area, pre-training on a large set of image caption pairs has led to highly effective multi-task models~\cite{Lu_2020_CVPR} as well as models that are incredibly capable at zero-shot classification~\cite{Radford2021LearningTV}. We investigate the question: Can pre-training help create effective multi-task embodied agents?


\begin{figure*}[tp]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/Fig1.pdf}
    \caption{We consider four high-level tasks that require navigation and object interaction. Skills are meaningful short sequences of primitive actions that are pre-trained and shared among tasks. On the right, we show an example of an episode by our multi-task agent for the long-horizon instruction following task of \emph{put a plunger in cabinet.} and an interactive question answering task of \emph{what color is plunger?}}
    \label{fig:teaser}
\end{figure*}

% Recent research has studied two forms of pre-training for E-AI: first, visual representation pre-training -- typically involves initializing the input CNN with an ImageNet pre-trained model~\cite{zhu2017target} or one trained on some classification task within the given simulated environment, and second, task pre-training -- typically involves pre-training the visual representation and controller for a long time period on a single task and then fine-tuning it for others~\cite{Wijmans2020DDPPOLN}. While the former method helps get training off the ground, it in itself is not the catalyst required to train generalizable multi-task agents. The latter is an effective approach when the downstream tasks are very similar to the pre-trained task, but is unlikely to generalize for diverse task sets.

In this paper, we propose a benchmark for multi-task E-AI with goal specified with natural language. The agents has to perform object navigation, exploratory interaction, instruction following and interactive question answering in photo realist environments with 110 object classes, 13 actions and continuous interaction parameterization. 
%
we propose a pre-training method for E-AI named Atomic Skill Completion (ASC) -- pre-train a low-level skill executing policy on a large set of atomic skills applicable to diverse downstream tasks, and then, train a high-level skill invocator on downstream tasks. ASC has several advantages over previous pretraining strategies: (1) Since ASC pre-trains on atomic skills instead of long-horizon downstream tasks, it pre-trains fairly quickly. (2) These skills are short horizon and relatively simple to learn and thus generalize better to unseen environments. (3) The atomic skills are chosen to be generic and can be chained to perform many downstream E-AI tasks. (4) Since high-level task invocation is now decoupled from low-level skill execution, the learning of high-level policies is hugely simplified, leading to the creation of effective multi-task embodied agents.

We pre-train our agent in the \thor environment on 9 atomic skills ranging from navigation skills such as \texttt{find X} to interactive skills such as \texttt{slice X} and the answering skill \texttt{answer}. We then jointly train the agent to perform 4 challenging tasks (Figure~\ref{fig:teaser}) -- (1) Short Horizon Instruction Following (\taskshort), (2) Long Horizon Instruction Following (\tasklong), (3) Interactive Question Answering (\taskiqa) and (4) Exploratory Interaction (\taskexp) and measure performance on Seen and Unseen environments. Given the interaction-heavy nature of these tasks, we consider two interaction modes -- \emph{Standard} whereby the agent must predict a bounding box that overlaps with the target object, and \emph{Hard} which requires the agent to accurately predict a point within the desired object. 

Our results show that pre-training the agent via \asc leads to improvements across all four tasks.
In the Standard setting for multi-task training, \asc improves Success Rates (averaged across all tasks) from 15.1 to 41.9 for Seen and 4.3 to 16.2 for Unseen; in the Hard setting, the improvements are as dramatic -- from 20.3 to 39.8 for Seen and 4.0 to 19.3 for Unseen. 
In the absence of pre-training, multi-task training results in a drop as compared to single task training for Unseen scenes (5.0 $\rightarrow$ 4.0), but when using \asc, multi-task training provides a large boost (10.9 $\rightarrow$ 19.3).
We also find that our multi-task agent with \asc performs comparably in the Hard setting vs the Standard setting -- 41.9 vs 39.8 Seen and 16.2 vs 19.3 Unseen, reflecting the ability of our agent to precisely predict the locations of target objects that it needs to interact with in the scenes. Finally, we find our model more interpretable than traditional Embodied AI solutions, since we can observe the sub-goals, target object and pixel locations for interaction output at each time step, enabling us to monitor progress and explain some successes and errors.

% Embodied AI researchers have long sought to develop agents that can perform complex tasks in visual environments -- tasks that require navigating around an environment and interacting with objects that lie within it. Much of the work in task completion has been studied in the context of instruction following, particularly low level and step by step instruction following, for instance: "Turn around and go up the stairs, turn right and go to right again towards the front door."

% While steady progress has been made in the domain of instruction following, such step by step detailed instructions are infrequently available in real world scenarios where an embodied agent may be required to complete a task. Step by step instructions assume an a priori knowledge of the scene layout and also assume a static layout of objects within the scene, assumptions that would prevent one from deploying an agent in novel environments or common everyday scenes where objects are moved around frequently by humans. Task completion using only end goal instructions, while more practical from a deployment standpoint, poses daunting challenges. Agents must be able to infer a series of short term actions such as \emph{MoveAhead}, \emph{TurnLeft} or \emph{PickUp} from long term goals such as \emph{"Heat the Potato"}, which is hard to learn. They must be able to fill in missing pieces of information via external knowledge or past experience, for instance, knowing that potatoes may be heated on a stove but must first be placed in a pan. And finally they must be capable of long horizon planning in the presence of uncertainty.

% Recent works in end goal instruction following have shown that end to end learning via imitation using moderately sized sets of expert trajectories simply does not work for complex tasks, and is poor at generalizing to not just new scenes but even new instructions within the training scenes \cite{alfred_leaderboard}. This is in sharp contrast to more constrained tasks like point goal navigation where end to end models trained with reward shaping perform exceedingly well. How can we bridge this huge and seemingly insurmountable gap in performance between these two tasks?

% Over the years many bodies of work have proposed variants of a highly intuitive idea -- train low level models to perform simple atomic skills, which we know can work pretty well, and then train a high level skill master policy that can invoke the appropriate sequence of skills given the end goal instruction. These works have often spanned grid worlds, low fidelity and simplistic visual environments, and frequently use templated language instructions -- assumptions that should make learning easier. And yet, while this idea is seemingly natural and has the benefits of being more interpretable than a black box model, improvements obtained over the vanilla end to end models tend to be surprisingly small (eg. roughly 10\% relative improvement on the task of EQA). As a result, the idea of a hierarchy of controllers has not quite taken off in popularity across Embodied AI.

% We revisit this idea in the challenging domain of ALFRED -- an instruction following dataset that requires agents to perform interactive tasks in photorealistic scenes using a series of low-level actions. But in contrast to past works evaluating on this benchmark, we only utilize the high-level end goal instruction and ignore the presence of step-by-step instructions. Inspired by the success of large scale pre-training in the vision, language and vision-and-language communities, we pre-train a skill-conditioned low level controller using a hugely diverse and large set of data-points using a combination of imitation learning and reinforcement learning. In an interactive environment, this requires obtaining expert trajectories via shortest paths not in a 2-D grid space, but in state space accounting for agent and object locations, interactions and object states. Our findings show that on the challenging ALFRED framework, scaling up skill pre-training massively and then using dynamic skill invocation is the key to getting the idea of hierarchical controllers to succeed. Importantly, it does not provide small fractional relative improvements but instead produces a massive improvement from XX to YY.

% These results using a tried, tested and often rejected technique are very promising. We hope that our strong results will encourage the community to revisit solutions that use explicit skill invocation. While single end-to-end models are becoming adept at solving atomic tasks, we posit that hierarchical and explicitly invoked controllers may be necessary to solve complex tasks going forward, particularly as we strive towards generalizing to new tasks and have a renewed focus on interpretability in the light of concerns around biases exhibited by our massive models.


% Introduce the complex interactive tasks -- useful agent can not only navigate but also interact with the environment. Provide two examples, Heat the apple or how many apples in the refrigerator.


% These high-level task is hard to collect and make them hard to generalize.


% 

% Contributions:
% Realistic setting for interactive embodied tasks. 

% High-level task datapoint is hard to obtain, we can pre-train each module in a robust and generalizable way. 

% The model learns discrete action and continuous interaction at the same time. 
% We showed high-level embodied tasks require more than Teacher Forcing. 
% Student Forcing and PPO (RL) methods play an essential role to learn a generalizable policy. 
% How to make SF and PPO works: 
% For hard tasks, the agent might be stuck at the beginning of the training and never explore the later stage. 
% How we solve this:
% Interaction radius annealing. 
% adaptive enforced planner when the error happens.  

==> sections/8_checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} We have provided details in the paper, as space permits and will provide more in supplementary along with code. 
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{} Due to our limited computational resources and the large number of experiments, we have not provided error bars for the submission unfortunately. However, we will provide errors bars for the main experiments for the final version.
    \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
    \end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
    \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> sty/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sty/space_saver.tex <==
% A collection of dubious space saving macros
\parskip=5pt
\abovedisplayskip 3.0pt plus2pt minus2pt%
\belowdisplayskip \abovedisplayskip
\renewcommand{\baselinestretch}{1} % only use this one in emergencies

%Section spacing
%Section spacing
\newcommand{\csection}[1]{
    \vspace{-0.11in}
    \section{#1}
    \vspace{-0.10in}
}

\newcommand{\csubsection}[1]{
    \vspace{-0.09in}
    \subsection{#1}
    \vspace{-0.08in}
}

\newcommand{\csubsubsection}[1]{
    \vspace{-0.06in}
    \subsubsection{#1}
    \vspace{-0.05in}
}

%caption/figure spacing
\setlength{\floatsep}{1ex plus 0ex minus 0.5ex}
\setlength{\textfloatsep}{3ex plus 0ex minus 0ex}
\setlength{\abovecaptionskip}{0ex plus 0ex minus 0ex}
\setlength{\belowcaptionskip}{0ex plus 0ex minus 0ex}
